Nearly-Optimal Consensus Tolerating Adaptive Omissions: Why is a Lot of Randomness Needed?

We study the problem of reaching agreement in a synchronous distributed system by $n$ autonomous parties, when the communication links from/to faulty parties can omit messages. The faulty parties are selected and controlled by an adaptive, full-information, computationally unbounded adversary. We design a randomized algorithm that works in $O(\sqrt{n}\log^2 n)$ rounds and sends $O(n^2\log^3 n)$ communication bits, where the number of faulty parties is $\Theta(n)$. Our result is simultaneously tight for both these measures within polylogarithmic factors: due to the $\Omega(n^2)$ lower bound on communication by Abraham et al. (PODC'19) and $\Omega(\sqrt{n/\log n})$ lower bound on the number of rounds by Bar-Joseph and Ben-Or (PODC'98). We also quantify how much randomness is necessary and sufficient to reduce time complexity to a certain value, while keeping the communication complexity (nearly) optimal. We prove that no MC algorithm can work in less than $\Omega(\frac{n^2}{\max\{R,n\}\log n})$ rounds if it uses less than $O(R)$ calls to a random source, assuming a constant fraction of faulty parties. This can be contrasted with a long line of work on consensus against an {\em adversary limited to polynomial computation time}, thus unable to break cryptographic primitives, culminating in a work by Ghinea et al. (EUROCRYPT'22), where an optimal $O(r)$-round solution with probability $1-(cr)^{-r}$ is given. Our lower bound strictly separates these two regimes, by excluding such results if the adversary is computationally unbounded. On the upper bound side, we show that for $R\in\tilde{O}(n^{3/2})$ there exists an algorithm solving consensus in $\tilde{O}(\frac{n^2}{R})$ rounds with high probability, where tilde notation hides a polylogarithmic factor. The communication complexity of the algorithm does not depend on the amount of randomness $R$ and stays optimal within polylogarithmic factor.

==> src/algorithm.tex <==
\section{Optimal Algorithm against Omissions Failures}
\label{sec:main-algo}
%\jo{This section has been rewritten, please let me know about any mistakes}
%\jo{The algorithm description is not easy to read. Adding some visual illustrations would be helpful.}
%TODO mention that our lower bound works for algorithms solving Consensus whp only while the algorithm below is correct always?
In this section, we present an algorithm that can solve Consensus with high probability in $O\left(\sqrt{n}\log^{2}{n}\right)$ rounds and uses $O\left(n^2 \log^4{n}\right)$ communication bits against any number $t < \frac{n}{192}$ of omission-faulty processes. The pseudocode of the algorithm is provided in Algorithm~\ref{alg:opt-omissions}.

The algorithm partitions processes into two classes: operative processes and \textit{inoperative} processes. The operative processes have the property that any two of them can exchange a bit of information in at most $O(\log{n})$ rounds, using a certain sparse graph of communication. In contrast, the inoperative processes are those that, due to the actions of the adversary, have been excluded from the fast flow of information guaranteed for the operative ones. The novelty of our approach is that the partition into operative and inoperative processes is not only dynamic, but also independent of the partition into faulty and non-faulty processes at the logical level. A non-faulty process may become inoperative if its communication neighborhood diminishes, while faulty processes may stay operative as long as they are good transmitters from the perspective of other processes, despite the omissions of some of their messages. The operative/inoperative status of a process is also local -- some other processes may not be aware of it.

To start, all processes are initially designated as operative (see line~\ref{line:operative-init}). Each operative process then selects a random sample of $\Theta(\log n)$ other processes, in expectation, to be its neighbors in the communication graph during the execution. Since this sampling is asymmetric, one round is allowed to inform the selected neighbors that they have been chosen. This results in each process having a set $V_p$ of processes with whom it will communicate during the protocol (see lines~\ref{line:graph_sampling}-\ref{line:rand-neigh}).

During the main loop of the algorithm (lines~\ref{line:main-for-begin}-\ref{line:main-for-end}), the operative processes work collectively to establish a consensus decision among them. This work is divided into $O(\sqrt{n}\log n)$ \textit{epochs} and utilizes a variant of the majority-vote protocols introduced for the case of, more benign, permanent crash failures in~\cite{Bar-JosephB98}.

The key novelty in our approach is that only operative processes participate in the majority-vote protocol adapted from~\cite{Bar-JosephB98}. This is achieved as follows: each operative process prepares a vote $b_p$ initialized to its input bit. In each epoch, the operative processes rely on two different communication subroutines, \textsc{GroupBitsAggregation} and \textsc{GroupBitsSpreading} (see lines~\ref{line:group-bits-aggr} and \ref{line:sum_ones_zeros}), to calculate the number of operative ones and zeros present in the votes. 
The efficient design of these communication algorithms constitutes another contribution of our paper.
%algorithm. 
Observe that during this communication, the adversary can arbitrarily fail processes, resulting in an uncontrolled shrinkage of the set of operative processes. Moreover, if the process of gathering votes was done naively, it would incur $\Omega(n^2)$ bit complexity per round, as potentially there are $n$ processes that want to communicate their vote to $n-1$ others (and since the required number of rounds is polynomial, as proved earlier in Theorem~\ref{thm:lower-randomness-res}, the communication complexity would be substantially above our goal of $\logO(n^2)$ communication bits). Nevertheless, the communication algorithms \textsc{GroupBitsAggregation} and \textsc{GroupBitsSpreading} overcome both these challenges and guarantee that every operative process has a correct estimation of the number of operative ones in the votes from the beginning of the epoch (the variable $\texttt{ones}_{p}$ in the pseudocode) and operative zeros in the votes from the beginning of the epoch (the variable $\texttt{zeros}_{p}$ in the pseudocode) after their completion. Since the description of these routines is highly technical, we devoted Subsection~\ref{subsec:comm-patterns} for this purpose.

Based on the values of the variables $\texttt{ones}_{p}$ and $\texttt{zeros}_{p}$ process $p$ decides what value to assign to variable $b_{p}$ for the next epoch. If the estimation $\texttt{ones}_{p}$ makes at least $\frac{6}{10}$ fraction of the estimation of all operative processes (which is 
%derive from 
equal to
$\texttt{ones}_{p} + \texttt{zeros}_{p}$), then the process assigns $b_{p} = 1$; if the estimation $\texttt{ones}_{p}$ is less than half of the 
%total 
estimation of the total number of operative processes then the process assigns $b_{p} = 0$. In any other case, it assigns $b$ to a uniform random bit. 

In the analysis, we will demonstrate that if the number of faulty or inoperative processes in a number of consecutive epochs is smaller than $\sqrt{n}$, the choices made by operative processes will lead to the same value $b$ across all of them with a constant probability. Our communication algorithms are designed in such a way that $\Theta(n)$ processes are always operative in the system, regardless of the adversary's actions. Therefore, after $O(\sqrt{n}\log{n})$ such epochs, we can assert that operative processes have reached a consensus decision (i.e., on same value) with high probability. 
%i.e., they store the same value as the vote.

In the last part of the algorithm, lines~\ref{line:good-spread}-\ref{line:final-receiv}, the operative processes broadcast their consensus value to all other processes. Then, every process that has received a vote acquires it and decides on the value of the vote. This part takes two rounds and $O(n^2)$ bits of communication. The formal analysis of the correctness, in particular, a thorough explanation of why operative processes are always a constant fraction of all processes, is given in Subsection~\ref{subsec:analysis-main}.
\begin{algorithm}[!h]
\SetAlFnt{\tiny}
\SetAlgoLined
\SetKwInput{Input}{input}
\Input{$\cP$, $p$, $b_p$}
$\texttt{operative}_{p} \leftarrow true$\;\label{line:operative-init}
$V_{p} \leftarrow$ a random subset of $\cP \setminus \{ p \}$ where each element is sampled independently with prob. $\frac{36\log{n}}{n - 1}$ \;\label{line:graph_sampling}
$p$ pings all processes $V_{p}$ and increments $V_{p}$ with all processes from which it has received a ping\;\label{line:rand-neigh}
$W_{1}, \ldots, W_{\ceil{\sqrt{n}}} \leftarrow $ a pre-defined partition of $\cP$ into 
$\ceil{\sqrt{n}}$ disjoint sets of size $\le \sqrt{n}$ each\;\label{line:sqrt-part}
let $\ell$ be such that $p\in W_\ell$\;\label{line:group}
\For{$\sqrt{n}\log(n)$ epochs\label{line:main-for-begin}}
{
$\texttt{g\_ones}_{p}, \texttt{g\_zeros}_{p}, \texttt{operative}_{p} \leftarrow \textsc{GroupBitsAggregation}(W_{\ell}, p,  \texttt{operative}_{p}; b_{p})$\label{line:group-bits-aggr}\;
\lIf{$\texttt{operative}_{p} = false$}{stay idle by the end of  line~\ref{line:good-spread}}

\BlankLine
$\texttt{ones}_{p}, \texttt{zeros}_{p},\texttt{operative}_{p} \leftarrow \textsc{GroupBitsSpreading}(V_{p}, p, \texttt{operative}_{p}; \texttt{g\_ones}_{p}, \texttt{g\_zeros}_{p})$\label{line:sum_ones_zeros}\;
\lIf{$\texttt{operative}_{p} = false$}{stay idle by the end of  line~\ref{line:good-spread}}

\BlankLine
\lIf{$\texttt{ones}_{p} > \frac{6}{10}(\texttt{ones}_{p} + \texttt{zeros}_{p})$}{$b_p \leftarrow 1$}\label{line:if-1} 
%\lElseIf{$\texttt{zeros}_{p} = 0$}{$b_p \leftarrow 1$}
\lElseIf{$\texttt{ones}_{p} < \frac{5}{10} (\texttt{ones}_{p} + \texttt{zeros}_{p})$}{$b_p \leftarrow 0$}\label{line:if-0}
\lElse{set $b_p$ to $0$ or $1$ with equal probability (independently at random)\label{line:if-random}}
}\label{line:main-for-end}
\lIf{$\texttt{operative}_{p} = true$}{\textbf{send} $b_{p}$ to all processes in $\cP$\label{line:good-spread}}
\lIf{any message $b_{q}$ from some process $q$ was received}{$b_{p} \leftarrow b_{q}$\label{line:final-receiv}}
\tcc{in the above, $q$ can be chosen arbitrarily from the received messages}
\Return{$b_{p}$}%\;
\caption{\textsc{OptimalOmissionsConsensus}}\label{alg:opt-omissions}
\end{algorithm}

\subsection{Communication patterns of operative processes within an epoch}\label{subsec:comm-patterns}
In this part we describe the communication algorithms used by processes to gather information about votes' distribution from the beginning of the epoch. We start by explaining the algorithm \textsc{GroupBitsAggregation}, which achieves the goal limited only to subgroups of processes of size $O(\sqrt{n})$. Limiting the size of a group on which we estimate the votes is crucial for achieving $O(n^2)$ communication bit complexity.\\
\noindent \textbf{Explanation of \textsc{GroupBitsAggregation}.} 
We partition the set of processes $\cP$ into at most $\ceil{\sqrt{n}}$ groups $W_{1}, \ldots, W_{\ceil{\sqrt{n}}}$, each with a size of at most $\sqrt{n}$ processes, as shown in lines~\ref{line:sqrt-part}-\ref{line:group}. Since every process knows the set of process names, the partition could be pre-defined, i.e., can be calculated locally by each process using the same local deterministic algorithm. Processes in different groups work independently in algorithm \textsc{GroupBitsAggregation}.

The objective of each group is to compute the number of operative processes within the group that have the variable $b$ set to $0$ and the number of those with $b = 1$, or mark inoperative the processes that cannot gather the necessary information. At the end of the algorithm, each operative process $p$ should have these two values, $\texttt{b\_zeros}_{p}$ and $\texttt{b\_ones}_{p}$, stored in its local memory, and updated its operative status $\texttt{operative}_{p}$. Algorithm~\ref{alg:bits-agreg} presents the pseudocode, while a formal description is provided below.
%%
For each group $W_{i}$, where $1 \le i \le \ceil{\sqrt{n}}$, we use a binary-tree decomposition of depth $\ceil{\log(\sqrt{n}))}$. At the lowest layer $L^{(i)}(1)$ of the decomposition, the processes in $W_{i}$ are divided into $\sqrt{n}$ singleton \textit{bags}, yielding the following:
$$L^{(i)}(1) := \{ L^{(i)}(1,1), \ldots, L^{(i)}(1, \sqrt{n}) \}.$$ 
For any subsequent layer $j$, $2 \le j \le \ceil{\log(\sqrt{n})}$, the bags of layer $j$ are formed as a union of bags at level $j-1$ corresponding to the children of the $j$-level bag in the tree. This way, at the higher levels of the decomposition, the number of bags is halved, but the size of a single bag is doubled. Formally, the bag $L^{(i)}(j, k)$, for $1 \le k \le \ceil{\frac{\sqrt{n}}{2^j}}$, which belongs to layer $L^{(i)}(j)$, is the union of bags $L^{(i)}(j - 1, 2k - 1)$ and $L^{(i)}(j - 1, 2k)$. Here, we assume that $L^{(i)}(j-1, k') = \emptyset$ if $k' \neq \ceil{\frac{\sqrt{n}}{2^{(j-1)}}}$.
%TODO add a picture of the tree here

The communication scheme is navigated by the structure described above. It proceeds in $\ceil{\log(\sqrt{n})}$ stages that correspond to aggregating knowledge within bags that belong to increasingly higher levels of the decomposition. 

In the first stage, each operative process $p$ that is a member of a bag $L^{(i)}(1, k)$ at the lowest layer $L^{(i)}(1)$ (for $1 \le k \le \sqrt{n}$) initializes two variables: $\texttt{b\_ones}_{p}(1,k)$ and $\texttt{b\_zeros}_{p}(1,k)$ that keep track of the value of its bit $b_{p}$, i.e., $\texttt{b\_ones}_{p}(1,k) = 1$ if $b_{p} = 1$, and $\texttt{b\_zeros}_{p}(1,k) = 1$ if $b_{p} = 0$ (see lines~\ref{line:if-operative-init}-\ref{line:if-inoperative-init}). Since at level $1$ the bags are singletons, every operative process has the correct number of one and zero votes of other operative processes in its bag.

In stage $j$, for $2 \le j \le \ceil{\log(\sqrt{n})}$ processes work to gather information of the votes of all other operative processes that belong to the same bag in the layer $L^{(i)}(j)$, see the main loop in line~\ref{line:main-for-group}-\ref{line:main-for-group-end}. For $1 \le k \le \ceil{\frac{\sqrt{n}}{2^j}}$, fix a bag $L^{(i)}(j, k)$ of the layer $L^{(i)}(j)$. By the hierarchical structure of the tree, at this point of the execution, the operative processes belonging to the left-child bag of $L^{(i)}(j, 2k - 1)$ already collected the number of operative $0$'s and $1$'s among them. The same is true for processes belonging to the right-child bag $L^{(i)}(j, 2k)$. 
To distribute this information between the operative processes in the bag $L^{(i)}(j, k)$, they use procedure $\textsc{GroupRelay}$ described below.\\
%%%

\begin{figure}
\centering
    \includegraphics[width=\textwidth]{focs23-submission/pictures/final-2.jpg}
    \caption{An explanation of the $3$-round communication dynamic in the \textsc{GroupRelay} procedure on an example of a set of four processes. On the left side of each round we have the binary-tree decomposition of a group of processes, on the right -- the same processes are depicted in their transmitters' role. The blue ellipsoid emphasis that processes work in the second layer to exchange the counts computed while considering the first layer (corresponding to leaves). Red processes are faulty, however, they are still participating in the protocol. Crossed process $p_{3}$ denotes the change of the state from operative to inoperative, after which $p_{3}$ is excluded from the role of a source.
    }
    \label{fig:group-relay}
\end{figure}
\noindent \textbf{Specification of the procedure \textsc{GroupRelay}.}
The procedure takes four inputs: the identifier of a process $p$ that executes it, its group $W_{i}$, the bag $L^{(i)}(j, k)$ 
%containing $p$, 
in which $p$ currently exchanges information, and the set $\texttt{counts}_{p}$, which is the information to be distributed among other operative processes in $L^{(i)}(j, k)$. The information could be initialized differently by the algorithm calling the procedure \textsc{GroupRelay}, depending on whether $p$ belongs to a left-child or a right-child of the bag $L^{(i)}(j, k)$ in the lower layer $j$, as shown in lines~\ref{line:group-relay-1}-\ref{line:group-relay-2} of Algorithm~\ref{alg:bits-agreg}.

During the execution of the procedure \textsc{GroupRelay}, the processes in $W_{i}$ have two different roles: \textit{non-faulty} processes of the entire group serve as \textit{transmitters}, while \textit{operative} processes in the bag $L^{(i)}(j, k)$ have an additional role of a \textit{source}. The following $3$-round protocol is executed. In the first round, each source sends its set $\texttt{count}$ to all transmitters. The transmitters collect received sets $\texttt{count}$ and prepare new sets of the same name $\texttt{count}$ that are the union of the former. There are at most four logically different values that processes (sources) of the bag $L^{(i)}(j,k)$ try to disseminate, which are the counts of operative zeros and ones originating in the two bags that are children of the bag $L^{(i)}(j,k)$ in the lower level of the decomposition. Therefore, each newly prepared set has a size of at most $O(\log{n})$ bits.
In the second round, the transmitters confirm to sources if they received a message in the previous round. Any source that receives less than $\frac{1}{2}|W_{i}| + 1$ confirmations becomes inoperative. In the third round, the transmitters send the new sets $\texttt{count}$ to the sources. Again, the sources that receive less than $\frac{1}{2}|W_{i}| + 1$ notifications in this round become inoperative. If a process becomes inoperative, it stops serving as a source, although it is still considered a potential transmitter in subsequent calls of the algorithm. The change in the operative status of a process is reported to the main algorithm \textsc{OptimalOmissionsConsenus} via variable $\texttt{operative}_{p}$. For an illustrative example, see Figure~\ref{fig:group-relay}.

After the procedure \textsc{GroupRelay} terminates, each process adds the received counts of operative ones and zeros and proceeds to the next stage of \textsc{GroupBitsAggregation}. Therefore, after the last stage, the operative processes gather the knowledge about the number of operative processes having $b=0$ and the number of those who have $b=1$ in the entire group $W_{i}$ (as this set corresponds to the bag being the root of the tree). These numbers are stored in variables $\texttt{b\_zeros}_{p}(\ceil{\sqrt{\log{n}}}, 1)$ and $\texttt{b\_ones}_{p}(\ceil{\sqrt{\log{n}}}, 1)$, and together with the operative status of a process, they are returned to the main algorithm \textsc{OptimalOmissionsConsenus}.
%%%

%TODO change the indexing in the code below
\begin{algorithm}
\SetAlFnt{\tiny}
\SetAlgoLined
\SetKwInput{Input}{input}
\Input{$W_{i}, p,  \texttt{operative}_{p}; b_{p}$}
\If{$\texttt{operative}_{p} = true$\label{line:if-operative-init}}
{
\lIf{$b_{p} = 0$} {$\texttt{b\_ones}_{p}(1, i) \leftarrow 0, \texttt{b\_zeros}_{p}(1, i) \leftarrow 1$}
\lElse{$\texttt{b\_ones}_{p}(1, i) \leftarrow 1, \texttt{b\_zeros}_{p}(1, i) \leftarrow 0$}
}
\lElse
{
$\texttt{b\_ones}_{p}(1, i) \leftarrow \perp, \texttt{b\_zeros}_{p}(1, i) \leftarrow \perp$
\label{line:if-inoperative-init}
}
\For{stage $j \in \{2, \ldots, \ceil{\log{n}}\}$\label{line:main-for-group}}
{
    let $L^{(i)}(j, k)$ be $p$'s bag in $j$-th layer $L^{(i)}(j)$\; 
    \lIf{$p \in L^{(i)}(j - 1, 2k - 1)$ \label{line:group-relay-1}}
    {
    $\texttt{counts}_{p} \leftarrow \{\texttt{b\_ones}_{p}(j - 1, 2k - 1), \texttt{b\_zeros}_{p}(j - 1, 2k - 1) \}$
    }
    \lElse{
        $\texttt{counts}_{p} \leftarrow \{\texttt{b\_ones}_{p}(j - 1, 2k), \texttt{b\_zeros}_{p}(j - 1, 2k) \}$ \label{line:group-relay-2}
    }
    $\texttt{counts}_{p}, \texttt{operative}_{p} \leftarrow \textsc{GroupRelay}(W_{i}, p, L^{(i)}(j,k), counts_{p})$\;
%    infer about 
extract values of variables $\texttt{b\_ones}_{p}(j - 1, 2k - 1), \texttt{b\_zeros}_{p}(j - 1, 2k - 1), \texttt{b\_ones}_{p}(j - 1, 2k)$, \ \ \ \ \ \ \ \ \ $\texttt{b\_zeros}_{p}(j - 1, 2k)$ based on the elements in the set $\texttt{counts}_{p}$\;
    $\texttt{b\_ones}_{p}(j, k) \leftarrow \texttt{b\_ones}_{p}(j - 1, 2k - 1) + \texttt{b\_ones}_{p}(j - 1, 2k)$\; 
    $\texttt{b\_zeros}_{p}(j, k) \leftarrow \texttt{b\_zeros}_{p}(j - 1, 2k - 1) + \texttt{b\_zeros}_{p}(j - 1, 2k) $
    \label{line:main-for-group-end}
}
\textbf{return} 
{$\texttt{b\_ones}_{p}(\ceil{\log{n}}, 1), \texttt{b\_zeros}_{p}(\ceil{\log{n}}, 1), \texttt{operative}_{p}$}\label{line:aggr-return}
%\;
\caption{\textsc{GroupBitsAggregation}\label{alg:bits-agreg}}
\end{algorithm}

\noindent \textbf{Explanation of \textsc{GroupBitsSpreading.}}
The algorithm \textsc{GroupBitsSpreading} serves as a tool to disseminate the values calculated by the grouped operative processes (in the run of the algorithm \textsc{GroupBitsAggregation}) to all operative processes.
%in disseminating to all operative processes the values that have been calculated by grouped operative processes in the run of the algorithm \textsc{GroupBitsAggregation}. 
The processes locally prepare an array of pairs $\texttt{BitPacks}$ of size $\ceil{\sqrt{n}}$ as follows. If $W_{\ell}$ is the group of a process in the partitioning $W_{1}, \ldots, W_{\ceil{\sqrt{n}}}$, then the process writes the numbers of operative processes of $W_{\ell}$ having $b = 0$ and having $b = 1$, which is the result of the algorithm \textsc{GroupBitsAggregation}, at the position $\ell$ of the array, keeping all other entries empty. 
Next, the communication is performed along links corresponding to the random graph sampled at the beginning of the execution, c.f., line~\ref{line:graph_sampling} of Algorithm~\ref{alg:opt-omissions}. Recall that the random graph is such that every process $p \in \cP$ decides whether to include another processes from $\cP$ as its neighbors, independently with probability $\frac{36\log{n}}{n - 1}$. Then, $p$ sends a prompt to selected processes letting them know that it has sampled them as neighbors. 
The set of selected processes and those who prompted $p$ is denoted $V_{p}$ and passed as a parameter to every execution of the algorithm \textsc{GroupBitsSpreading}.

The communication in the \textsc{GroupBitsSpreading} algorithm lasts $4\log{n}$ rounds. Initially, $p$ sends to every process in $V_{p}$ the entries of the array $\texttt{BitPacks}_{p}$ that have not been sent via the link yet. When receiving a message from another process $q \in V_{p}$ process $p$ updates its array $\texttt{BitPacks}_{p}$ by replacing empty entries with the non-empty entries of the array $\texttt{BitPacks}_{q}$. Additionally, $p$ keeps track of the processes from $V_{p}$ who failed to deliver a message in the most recent round and excludes them from the communication and refutes to accept messages from them in any future round of the algorithm \textsc{GroupBitsSpreading}. %\dk{??? globally, or only future rounds of \textsc{GroupBitsSpreading} ???} 
If the number of processes from which $p$ received a message is less than $\log{n}$, $p$ becomes inoperative. It stays idle to the end of the current epoch and in all future epochs of the execution of the main algorithm \textsc{OptimalOmissionsConsensus}. 

After $4\log{n}$ rounds, each operative process adds up the values in its array $\texttt{BitPacks}$ corresponding to the numbers of $0$'s and $1$'s, resp., in different groups, and returns these two numbers. The key property, which we prove formally in the analysis of the protocol, is that any two values returned by the operative processes (either the count of $0$'s or $1$'s) may differ by at most the number of processes that have turned inoperative during the epoch. 

\begin{algorithm}
\SetAlFnt{\tiny}
\SetAlgoLined
\SetKwInput{Input}{input}
\Input{$V_{p}, p, \ell, \texttt{operative}_{p}; \texttt{g\_ones}_{p},\texttt{g\_zeros}_{p}$}
%\texttt{g\_zeros}_{p}, \texttt{g\_ones}_{p}$}
$\texttt{BitPacks}_{p} \leftarrow [(\emptyset, \emptyset), \ldots, (\emptyset, \emptyset)]$, an array of pairs (initially of zeros) of size $\ceil{\sqrt{n}}$\;
$\texttt{BitPacks}_{p}[\ell] \leftarrow (\texttt{g\_ones}_{p}, \texttt{g\_zeros}_{p})$\;
\For{$4\log{n}$ rounds}
{
    \textbf{for} $q \in V_{p}$ : \newline
    \hspace*{2.5mm} \textbf{send} a message containing $\texttt{BitPacks}_{p}$ to $q$, if $q$ not disregarded before\newline
    \hspace*{2.5mm} \textbf{receive} a message (if any) with $\texttt{BitPacks}_{q}$ sent by $q$:\newline
    \hspace*{5mm} \textbf{if} $q$ has not sent a message, disregard sending to $q$ in any future round;\newline
    \hspace*{5mm} \textbf{for} $i \in [\ceil{\sqrt{n}}]$ :  %\textbf{ do } 
    $\texttt{BitPacks}_{p}[i] \leftarrow \texttt{BitPacks}_{p}[i] \vee \texttt{BitPacks}_{q}[i]$\;\label{line:spreading-comm}
    \lIf{number of received messages is less than $\log{n}$}{\newline \hspace*{2.5mm} $\texttt{operative}_{p} \leftarrow false$;\newline \hspace*{2.5mm} stay idle until line~\ref{line:spread-return}}
}
$\texttt{ones}_{p}, \texttt{zeros}_{p} \leftarrow $ the sum of the first (or the second resp.) elements of each non-empty pair of $\texttt{BitPacks}_{p}$\;
\textbf{return} $\texttt{ones}_{p}, \texttt{zeros}_{p}, \texttt{operative}_{p}$\label{line:spread-return}
%\;
\caption{\textsc{GroupBitsSpreading}\label{alg:bits-spread}}
\end{algorithm}

%Similar ideas have been considered in the literature, c.f.~\cite{Bar-JosephB98}, who showed how values $b$ converge within an execution, with a similar asymptotic, within the set of non-faulty processes. Despite improved communication, ours generalizes the process of converging of values $b$ to the set of operative processes, that can be in arbitrary relation with the set of faulty processes. \dk{??? I don't understand the last sentence ???}


\subsection{Analysis}\label{subsec:analysis-main}
Building blocks of an execution of the algorithm are \textit{epochs} -- full iterations of the main loop of the algorithm \textsc{OptimalOmissionsConsensus}. 
%Recall, that a process $p$ is \textit{operative} (at some point of the execution) if it satisfies $\texttt{operative}_{p} = true$ at this point of the execution. 
As any final decision of a process comes from a communication with an operative process, see line~\ref{line:final-receiv}, our goal is to prove that after all epochs, with large probability, the operative processes store the same value in their variables $b$. 
To achieve that, we will gradually analyze how consecutive subroutines executed within an epoch influence the values $b$ held by operative processes.\\
\noindent \textbf{Analysis of} \textsc{GroupBitsAggregation} \textbf{algorithm.}
In this algorithm, the operative processes work in groups that are given by the partition $\{ W_{1}, \ldots, W_{\ceil{\sqrt{n}}}\}$ of the set $\cP$.
Consider a group $W_{i}$.  For a process $p$ and a process $q$ such that $p, q$ in $W_{i}$, we say that $q$ \textit{contributes} to variable $\texttt{b\_ones}_{p}(j, k)$ $(\texttt{b\_zeros}_{p}(j, k)$ respectively), for some $j \in [\ceil{\log(\sqrt{n})}]$, $k \ge 0$, if the input $b_{q}$ is counted in the variable $\texttt{b\_ones}_{p}(j, k)$ (or $(\texttt{b\_zeros}_{p}(j, k)$ depending on the value of $b_{q}$). 

\begin{lemma}\label{lem:bits-agg-contr}
Let $M_{i} \subseteq W_{i}$ be the set of operative processes in the group $W_{i}$ at the end of the algorithm \textsc{GroupBitsAggregation}.
Any process $q \in M_{i}$ contributes consistently to both variables, $\texttt{b\_ones}_{p}(\ceil{\log(\sqrt{n})}, 1)$ and $\texttt{b\_zeros}_{p}(\ceil{\log(\sqrt{n})}, 1)$, of any other process $p \in M_{i}$.
\end{lemma}

\begin{proof}
The proof proceeds by induction on the depth of a layer in the tree decomposition $L^{(i)}$ of the group $W_{i}$. For the base case, we observe that the lemma holds for any pair of processes belonging to the set $M_{i} \cap L^{(i)}(1, k)$, where $L^{(i)}(1, k)$ is a bag in the first layer, simply because $M_{i} \cap L^{(i)}(1, k)$ is a singleton set.

For the inductive step, consider a bag $L^{(i)}(j, k)$ in some layer $j > 1$. Let $p$ and $q$ be any two processes belonging to $M_{i} \cap L^{(i)}(j, k)$. During the execution of the $\textsc{GroupRelay}$ procedure, the process $p$, who had the role of a source, relayed its set $\texttt{count}$ to at least $\frac{1}{2}|W_{i}| + 1$ other processes (transmitters), because otherwise it would have lost its operative status. Similarly, $q$ has received the accumulated set $\texttt{count}$ from at least another $\frac{1}{2}|W_{i}| + 1$ processes. However, these two sets of transmitters must have at least one common transmitter, who in this case assures that $q$ received the counts of $p$ (or other counts corresponding to the bag of $p$ on the layer $j - 1$, but those are equivalent based on the inductive hypothesis). Since $L^{(i)}(1, 1) = W_{i}$, the lemma is proven.
%
\end{proof}

Next, we bound the bit complexity of the algorithm $\textsc{GroupBitsSpreading}$ when limited to a single group only.

\begin{lemma}\label{lem:msg-aggr}
Processes in a single group use at most $O(n\log^2{n})$ bits of communication, in total, in an execution of the algorithm $\textsc{GroupBitsAggregation}$.
\end{lemma}

\begin{proof}
The algorithm takes $O(\log{n})$ stages of communication. In a stage, the procedure $\textsc{GroupRelay}$ is executed to distribute information between processes belonging to every bag of the layer of the stage. The information about a single bag distributed in the messages of the procedure $\textsc{GroupRelay}$ is of size $O(\log{n})$ bits at most, as it contains at most four counts of size $O(\log{n})$ each, c.f. the description of the procedure. The messages send in the procedure are always between transmitters and sources. This first class of processes contains at most $O(\sqrt{n})$ processes (the size of any group). The second amortizes to $O(\sqrt{n})$ if considered the union of all bags on the layer corresponding to the stage. It follows then, that at most $O(n)$ messages is sent per stage, in total. Thus the lemma follows.
\end{proof}

\noindent \textbf{Analysis of} \textsc{GroupBitsSpreading} \textbf{algorithm.}
We first explain formally the scheme of communication used in the algorithm \textsc{GroupBitsSpreading}.
Let $\cR(n, \rho)$ be a random graph on $n$ vertices in which every edge is contained independently with probability $\rho$. 
Let $G$ be a graph with vertices corresponding to the set of processes $\cP$ and edges defined by the random experiment in line~\ref{line:rand-neigh} of \textsc{OptimalOmissionsConsensus} algorithm. That is, an edge $(p_{1},p_{2})$, for $p_{1}, p_{2} \in \cP$, belongs to $G$ if either $p_{1} \in V_{p_{2}}$ or $p_{2} \in V_{p_1}$. Because each process samples the set $V$ as a random subset of $\cP$ such that each element is contained independently with probability $\frac{36\log{n}}{n- 1}$, therefore edges of $G$ appears independently with probability $1 - \left(1 - \frac{36\log{n}}{n - 1}\right)^2$. 
\begin{observation}\label{obs:g-is-random}
$G$ is an instance of a random graph $\cR(n, \rho)$, where 
$$\rho := 1 - \left(1 - \frac{36\log{n}}{n - 1}\right)^2 \ge \frac{36\log{n}}{n - 1}.$$
\end{observation}
\noindent Note here that the graph $G$ as a whole is unknown to processes who have only their local view on it -- the set of their neighbors. 
%TODO change delta below
Next, we focus on certain known properties of random graphs. For suitable parameters $\alpha$, $\beta$, $\delta$~and~$\ell$, the following properties will be used to analyze omission-tolerance of the random graph $G$. 
\begin{definition}[\textit{of expansion, edge-density, and compactness}]
\hfill
\begin{itemize}
    \item \textbf{Expansion:} graph~$G$ is said to be  \emph{$\ell$-expanding}, or to be an \emph{$\ell$-expander}, if any two subsets of~$\ell$ nodes each are connected by an edge. 
   
    \item \textbf{Edge-density:} graph~$G$ is said to be \emph{$(\ell,\alpha,\beta)$-edge-dense} if, for any set $X\subseteq V$ of \emph{at least} $\ell$ nodes, there are at least $\alpha |X|$ edges internal for~$X$, and for any set $Y\subseteq V$ of \emph{at most} $\ell$ nodes, there are at most $\beta |Y|$ edges internal for~$Y$.
        
    \item \textbf{Compactness:}
    graph~$G$ is said to be \emph{$(\ell,\varepsilon,\delta)$-compact} if, for any set $B\subseteq V$ of at least $\ell$ nodes, there is a subset $C \subseteq B$ of at least $\varepsilon\ell$ nodes such that 
    each node's degree in~$G|_C$ is at least~$\delta$. We call any such set~$C$ a \emph{survival set for~$B$}.
\end{itemize}
\end{definition}
To assure that the random graph $G$ used in the algorithms satisfies the above properties with high probability, we reuse the following theorem. 
%TODO precise the lemma below, esp (n / 192)

%\dk{??? We need to correct PODC citations below ???}

\begin{theorem}[Theorem $2$ in~\cite{ChlebusKS-PODC09}]
\label{thm:random-graph-properties}
Let $n \in \textbf{N}$, %$k := \frac{2}{3}n$ 
and $\Delta' \ge \Delta = 36\log{n}$. A random graph $\cR(n, \Delta' / (n - 1))$ satisfies all the below properties whp:\\
\noindent  
	\emph{(i)} it is $(n/192)$-expanding, 
\hspace*{6.4em}
	\emph{(ii)} it is $(n/96,3/4,\Delta/36)$-compact, 

\noindent	\emph{(iii)} it is $(n/96,\Delta/8,\Delta/144)$-edge-dense,
\hspace*{0.5em}
\emph{(iv)} the degree of each node is between $33\Delta$ and $39\Delta$.
	
%\noindent	\emph{(v)} if $\lambda_{1} \ge \lambda_{2} \ge \ldots \ge \lambda_{n}$ are eigenvalues of its normalized adjacency matrix, then $|\max(\lambda_{2}, \lambda_{n}) | \le \frac{1}{\sqrt{\delta}}.$\footnote{https://web.mit.edu/18.338/www/2012s/projects/yz\_slides.pdf}
\end{theorem}

By Observation~\ref{obs:g-is-random}, $G$ has been constructed as a random graph $\cR(n, \rho)$, for $\rho \ge \frac{36\log{n}}{n - 1}$, thus it satisfies the assumption of Theorem~\ref{thm:random-graph-properties} and possesses all the above properties whp. 
As a consequence of these properties, it can be also shown that close neighborhoods of any vertex in $G$ contain regular subgraphs and grow rapidly. Let us start by giving the appropriate definition.

\begin{definition}[\textit{of $(\gamma,\delta)$-dense-neighborhood}]
For a node $v\in V$, a set $S\subseteq N^{\gamma}_G(v)$  is said to be \emph{$(\gamma,\delta)$-dense-neighborhood for~$v$} if each node in~$S\cap N^{\gamma-1}_G(v)$ has at least $\delta$ neighbors in~$S$.
\end{definition}

To formalize the meaning of the rapid growth of a close neighborhood of a vertex in $G$, consider the following lemma.

\begin{lemma}[Lemma $1$ in~\cite{ChlebusKS-PODC09}] \label{lemma:sparse-to-dense}		
If graph~$G=(V,E)$ of $n$ nodes is $(n/96,\delta/8,\delta/144)$-edge-dense then any $(r,\delta/36)$-dense-neighborhood for a node $v\in V$ has at least $\min\{2^{r}, n/96\}$ nodes, for $r \ge 0$.
\end{lemma}
%We can also show that graphs satisfying properties of Theorem~\ref{thm:random-graph-properties} are dense enough to assure that a large fraction of processes remain operative regardless of the adversary actions.

\noindent Establishing the necessary properties of the communication graph used in runs of the \textsc{GroupBitsSpreading} algorithm, we focus on analyzing how information is spread across the graph in these runs. 
Recall, that we focus our attention only on these actions that happen within a single epoch -- a single iteration of the loop in the main algorithm~\textsc{OptimalOmissionsConsensus}. For an epoch, let $\texttt{OP\_END}$ denote the set of these processes that are operative at the end of the epoch. 
We say that a process $p \in \texttt{OP\_END}$ can \textit{reach} a process $q \in \texttt{OP\_END}$ during the run of the algorithm \textsc{GroupBitsSpreading}, if there exists a path of processes $p = s_{1}, s_{2}, \ldots, s_{k} = q$, such that the process $s_{i + 1}$ received a message from $s_{i}$ in $i$th round of the run of the \textsc{GroupBitsSpreading} algorithm, for any $1 \le i \le k - 1$.

\begin{lemma}\label{lem:spreading-reaching}
For any two processes $p, q \in \texttt{OP\_END}$ it holds that $p$ can reach $q$.
\end{lemma}

\begin{proof}
%%%Revise the below proofs grammatically...
%TODO Polishing the proof.
Consider the following inductive construction. For the base case, let $B_{0} = {p}$, and define $R^{0}(p)$ the set of these processes from which $p$ received a message in the last iteration of the main loop of \textsc{GroupBitsSpreading}. Then define a \textit{graph} $B_{1}$ (which is a subgraph of $G$) with the set of vertices being $B_{0} \cup R^{0}(p)$ and the set of edges being the link by which $p$ received a message from $R^{0}(p)$ in the last round of the loop. 
First, $|R^{0}(p)|$ is at least $\log{n}$ since $p$ remained operative to the end of the main loop of the algorithm. Therefore, the graph $B_{1}$ satisfies the definition of $(1, \log{n})$-dense-neighborhood of $p$. 
Second, the links corresponding to edges of the graph $B_{1}$ have been continuously relaying messages in both directions for the first $4\cdot \log{n} - 1$ rounds of this loop. This follows from the fact, that a process sends a message only to a process from which it has been receiving a message prior to the send instruction, see line~\ref{line:spreading-comm} in the algorithm \textsc{GroupBitsSpreading}. 
Third, processes corresponding to vertices of $B_{1} = \{p\} \cup R^{0}(p)$ have been operative for the first $4\cdot \log{n} - 1$ rounds of the loop, since only operative processes participate in the communication.

We inductively define the set $R^{i}(p)$, for $1 \le i \le \log{n}$, as a set of these processes that sent a message to processes corresponding to vertices in $B_{i}$ in the round $4\cdot \log{n} - i$ of the main loop. 
Then, the graph $B_{i + 1}$ is defined. The vertices of $B_{i+1}$ are processes from $R^{i}(p) \cup B_{i}$, while edges are derived from the edges of $B_{i}$ and these links that correspond to the communication between $R^{i}(p)$ and $B_{i}$ in the round $4\cdot \log{n} - i$. 
By the inductive assumption, processes from $B_{i}$ were operative for the first $4\cdot \gamma - \log{n}$ rounds. Therefore, in round $4\cdot \log{n} - i$ each of them received at least $\log{n}$ messages, which yields that the graph $B_{i + 1}$ is $(i + 1, \log{n})$-dense-neighborhood of $p$. 
The fact that processes only send messages to those processes from whom they have been continuously receiving messages, assures that links corresponding to edges of $B_{i + 1}$ propagated messages in both directions for the first $4\cdot\log{n} - (i + 1)$ rounds of the analyzed loop. Finally, all processes from $B_{i + 1}$ were operative for the first $4\cdot\log{n} - (i + 1)$ rounds as they sent a message in the round $4\cdot\log{n} - i$ of the main loop. This completes the inductive construction.

Consider now the set $B_{\log{n}}$. First, it is a subgraph of $G$, and by the above reasoning, it is a $(\log{n}, \log{n})$-dense-neighborhood of $p$. By Lemma~\ref{lemma:sparse-to-dense}, we conclude that the size of $B_{\log{n}}$ is at least $\frac{n}{96}$. By the inductive construction above, all processes corresponding to vertices in $B_{\log{n}}$ are in distance $\log{n}$ at most from $p$. Moreover, all links corresponding to the edges of $B_{\log{n}}$ correctly relayed messages in \textit{both} directions for the first $4\log{n} - \log{n} = 3\log{n}$ rounds of the main loop of the algorithm \textsc{GroupBitsSpreading}. As a consequence, $p$ can reach any other vertex (equivalently process) from $B_{\log{n}}$ and any other vertex (equivalently process) from $B_{\log{n}}$ can reach $p$ (as the communication is bidirectional in $B_{\gamma}$).

Let us construct the analogous set, $B'_{\log{n}}$ for the process $q$, relying on its operational status. The same reasoning as above gives us that $|B'_{\log{n}}| \ge \frac{n}{96}$ and that any process from $B'_{\log{n}}$ reaches and can by reached by $q$. 
Since there is at most $\frac{n}{192}$ faulty processes in the system, the parts of sets $B_{\gamma}$ and $B'_{\gamma}$ consisting of only non-faulty processes, are of size $\frac{n}{192}$ each, and thus are connected by at least one edge. The last follows from the $(n/192)$-expanding property of $G$. 
It then follows, that $p$ can reach $q$ by a path of length $2\log{n} + 1$ at most, and since all links corresponding to edges from both $B_{\log{n}}$ and $B'_{\log{n}}$ worked correctly for the first $3\log{n}$ round of the main loop, the lemma is proven. 
\end{proof}

\noindent \textbf{Analysis of the main algorithm}.
In the final part of the proof, we connect together the properties of the algorithms \textsc{GroupBitsAggregation} and \textsc{GroupBitsSpreading} and explain how they lead to correct updates of values $b$ in lines~\ref{line:if-1}-~\ref{line:if-random} of the main algorithm~\textsc{OptimalOmissionsAlgorithm}, resulting eventually in a consesus decision.   
We start by noting that the communication graphs used in any of the inner algorithms are dense enough to maintain a large fraction of correct processes operative, regardless of the actions of the adversary. Recall also the assumption that the number $t$ of faulty processes is less than $\frac{n}{192}$.
%\jo{
\begin{lemma}\label{lem:good-proc-are-large}
For any epoch, the size of the set $\texttt{OP\_END}$ is always larger than $\frac{47}{64}n$.
\end{lemma}
\begin{proof}
Consider any epoch $\cE$ of the algorithm and recall the partition $\{ W_{1}, \ldots, W_{\ceil{\sqrt{n}}}\}$ of the set $\cP$  used in the algorithm $\textsc{GroupBitsAggregation}$. Since the adversary can fail at most $\frac{n}{192}$ processes than by a counting argument there exists a set of $\sqrt{n} - \frac{1}{96}\sqrt{n}$ groups, which corresponds to a set of at least $\frac{95}{96}n$ processes, such that every process in the set has more than half non-faulty processes in its group. Let $X$ be a subset of the previous set consisting only of non-faulty processes. We have that $|X| \ge \frac{95}{96}n - \frac{1}{192}n \ge \frac{94}{96}{n}$.
Consider now the subgraph induced by $X$ in the random graph $G$ used for the communication in $\textsc{GroupBitsSpreading}$ algorithm. Using $(n/96, 3/4, \log{n})$-compactness property of $G$ (c.f. Theorem~\ref{thm:random-graph-properties}), we conclude that there exists $X' \subseteq X$ that has size at least $\frac{3}{4} \cdot |X| \ge \frac{3}{4}\frac{94}{96}n = \frac{47}{64}n$ and such that every process from $X'$ has degree at least $\log{n}$ in $X'$. 
We finish the proof by observing, that no process from $X'$ could become inoperative in any epochs earlier than $\cE$. First, every process $p$ from $X'$ belongs also $X$ thus, as observed above, it always receives more than half of messages from its group in all executions of \textsc{GroupBitsAggregation} that have occurred before $\cE$. Second, we choose $X'$ to consist only of non-faulty processes. Communication between them is then always reliable and together with the property that every process of $X'$ is of degree $\log{n}$ at least in $X'$, we see that they always stay operative in the course of executions of algorithm \textsc{GroupBitsSpreading}.
\end{proof}
%}
We say that a process $p$ \textit{contributes} to the sum of ones (or zeros) of a process $q$ if its bit $b_{p}$ is included in the value $ones_{q}$ calculated in line~\ref{line:sum_ones_zeros} of the main algorithm~\textsc{OptimalOmissionsConsensus} ($zeros_{q}$ resp.). 
\begin{lemma}\label{lem:operative-contribution}
For any epoch, every process $p$ contained in the set $\texttt{OP\_END}$ with $b_{p} = 1$ contributes to the sum of ones of any other process $q$ from $\texttt{OP\_END}$. Analogically, if $b_{p} = 0$ then $p$ contributes to the sum of zeros of any other process $q$ from $\texttt{OP\_END}$.
\end{lemma}
\begin{proof}
Consider any $p \in \texttt{OP\_END}$. Let $W_{i}$ be the $p$'s group, i.e. $p \in W_{i}$. 
By Lemma~\ref{lem:bits-agg-contr}, we get that any operative process $r$ contributes to the values returned any other operative process in the algorithm \textsc{GroupBitsAggregation}.
This yields, that whatever pair of values  $(\texttt{g\_ones}_{i}, \texttt{g\_zeros}_{i})$, describing the number of $0$'s and $1$'s among operative process in $W_{i}$, the process $q$ receives during the execution \textsc{GroupBitsSpreading} algorithm, the bit value $b_{p}$ contributes to this pair. 
On the other hand, Lemma~\ref{lem:spreading-reaching} assures that $p$ can reach $q$. 
It follows that $q$ receives at least one pair of values $(\texttt{g\_ones}_{i}, \texttt{g\_zeros}_{i})$, and the lemma is proven.
\end{proof}


\begin{lemma}[Lemma $4.3$ in~\cite{Bar-JosephB98}]\label{lem:anti-concetration}
Assume that $n$ processes independently choose a random bit from uniform distribution. Let $x$ be the random variable denoting the processes that chose bit $1$. Then for any $t \le \sqrt{n} / 8$
$$\Pr(x - \E(x) \ge t\sqrt{n}) \ge \frac{e^{-4(t+1)^2}}{\sqrt{2\pi}} \ .$$
\end{lemma}


\noindent We call an epoch \textit{good} if at most $\sqrt{n}$ processes become inoperative during the epoch. The following explains how lines~\ref{line:if-1}-~\ref{line:if-random} change $b$ values of operative processes under the assumption of a sequence of consecutive good epochs. 
\begin{lemma}\label{lem:three-epochs}
Consider three consecutive good epochs $\cE_{1}, \cE_{2}, \cE_{3}$. Let $\texttt{OP\_END}_{3}$ be the set of operative processes at the end of the epoch $\cE_{3}$. 
Then with probability $\Omega(1)$ all processes belonging to $\texttt{OP\_END}_{3}$ store the same value $b$ before the third epoch ends.
\end{lemma}
\begin{proof}
Let $\texttt{OP\_END}_{1}$ be the set of these processes that are operative when line~\ref{line:if-random} is executed during the epoch $\cE_{1}$. Using Lemma~\ref{lem:good-proc-are-large}, we have that $|\texttt{OP\_END}_{1}| \ge \frac{47}{64}n$. Combining Lemma~\ref{lem:operative-contribution} with the assumption that in the epoch $\cE_{1}$ at most $\sqrt{t}$ change their status to inoperative, we see that values $ones_{p}$, $zeros_{p}$ and $ones_{p} + zeros_{p}$ calculated in a process $p$ in epoch $\cE_{1}$ differ by at most $\sqrt{t}$ from the corresponding values of any other processes from $\texttt{OP\_END}_{1}$. 
Therefore, in the epoch $\cE_{1}$ no two processes can execute line~\ref{line:if-1} and line~\ref{line:if-0} at the same time, since the difference between right-hand-sides of these two inequalities is at least $\frac{1}{10}|\texttt{OP\_END}_{1}| > \sqrt{t}$.

We first consider the case when no process executes line~\ref{line:if-0}. In such a scenario, processes either assign a random bit to $b$ or the value $0$. Nevertheless, by Lemma~\ref{lem:anti-concetration}\footnote{Although Lemma~\ref{lem:anti-concetration} concerns the number of $1$'s being chosen by processes, if the distribution is uniform then $0$ and $1$ have the same probability of occurring and, by the symmetry, the same lemma can be used to estimate the number of chosen $0$'s.} with a constant probability $C_{1}$, the number of processes starting the next epoch $\cE_{2}$ with $b$ equal zero is at least $\frac{|\texttt{OP\_END}_{1}|}{2} + 3\sqrt{t}$. It follows that the number of processes having $b = 1$ is at most
$$|\texttt{OP\_END}_{1}| - \frac{|\texttt{OP\_END}_{1}|}{2} - 3\sqrt{t} \le \frac{|\texttt{OP\_END}_{1}|}{2} - 3\sqrt{t}.$$
In the epoch, $\cE_{2}$ at most $\sqrt{t}$ processes become inoperative and thus the ratio of the number of $1$'s held by the operative processes to the total number of operative processes must remain lower than $\frac{1}{2} = \frac{5}{10}$ in the entire epoch $\cE_{2}$. It follows then, that all operative processes execute line~\ref{line:if-0} and assign $b$ to $0$ before the epoch ends. 

The second case is when at least one process execute line~\ref{line:if-1} in the epoch $\cE_{1}$. Let $x$ be the number of processes that in this epoch execute line~\ref{line:if-random}. We proceed in two subcases:
\begin{itemize}
    \item Assume that $x \ge \frac{8}{10}|\texttt{OP\_END}_{1}|$. By Lemma~\ref{lem:anti-concetration}, with a constant probability $C_{2}$, more than $\frac{4}{10}|\texttt{OP\_END}_{1}| + 3\sqrt{t}$ from processes who executed line~\ref{line:if-random} assign $0$ to their value $b$. It follows then that at the beginning of the epoch $\cE_{2}$ at most
    $$|\texttt{OP\_END}_{1}| - \frac{4}{10}|\texttt{OP\_END}_{1}| + 3\sqrt{t} < \frac{6}{10}|\texttt{OP\_END}_{1}| - 3\sqrt{t}$$
    processes have value $b$ assign to $1$. Since in $\cE_{2}$ at most $\sqrt{t}$ processes become inoperative. Therefore, we arrived at the case when no process can execute line~\ref{line:if-1} in the current epoch and the two next epochs are good. Using the same logic as for the first case of this lemma, we get that with a constant probability $\Omega(1)$ all operative processes will have value $b$ equals $0$ before the third epoch ends.
    \item Suppose that $x < \frac{8}{10}|\texttt{OP\_END}_{1}|$. By Lemma~\ref{lem:anti-concetration} there is a constant probability that at most $\frac{4}{10}|\texttt{OP\_END}_{1}| - 3\sqrt{t}$ processes who change $b$ randomly assign $0$ as its value. Therefore, at least
    $$|\texttt{OP\_END}_{1}| - \frac{4}{10}|\texttt{OP\_END}_{1}| + 3\sqrt{t} = \frac{6}{10}|\texttt{OP\_END}_{1}| + 3\sqrt{t}$$
    processes start the subsequent epoch $\cE_{2}$ with $b$ set to $1$. Since in the epoch $\cE_{2}, $ at most $\sqrt{t}$ changes of the operative status occur and Lemma~\ref{lem:operative-contribution} proves that operative processes get their values $b$, thus all operative processes must execute line~\ref{line:if-1} in the epoch $\cE_{2}$ and therefore assign value $1$ to their variable $b$.
\end{itemize}
\end{proof}

%\jo{
\noindent Finally, we give the main theorem.
\begin{theorem}
\label{thm:main-algo}
The algorithm \textsc{OptimalOmissionsConsensus} solves Consensus against an adaptive adversary capable of controlling $t < \frac{n}{192}$ processes in $O\left(\sqrt{n} \log^{2}(n)\right)$ rounds, uses $O\left(n^2 \log^{4}n\right)$ communication bits and $O\left(n^{3/2}\log^2{n}\right)$ random bits, whp.
\end{theorem}
\begin{proof}
We first prove correctness.
If all processes start with the same bit value, either $0$ or $1$, then with probability $1$ all operative processes carry the same bit value (consistent with the initial bit) of the variable $b$ throughout all epochs, since the processes throughout the execution manipulate only on the input bits. Observe, that in such case no process ever accesses a random source in line~\ref{line:if-random} of the algorithm \textsc{OptimalOmissionsConsensus}, as the ratio of $1$'s of operative processes to all values is always either $0$ or $1$.

If the processes' inputs are mixed then the following holds. By Lemma~\ref{lem:good-proc-are-large}, there are at most $\frac{17}{64}n$ processes that might become inoperative during the run of the algorithm. On the other hand, any epoch that is not good has at least $\sqrt{n}$ processes that become inoperative. Since the algorithm executes $\sqrt{n}\log(n)$ epochs, thus by the pigeonhole principle there is at least $\Omega(\log{n})$ disjoint triples of consecutive \textit{good} epochs. By Lemma~\ref{lem:three-epochs}, after each such triple, there is a $\Omega(1)$ probability that all operative processes have the same value of the variable $b$. Observe, also that by a similar argument as above, if operative processes start an epoch with the same bit, the bit remains their choice of value $b$ in the following epoch as well. Again, this is derived from the fact that in such case no operative processes can access line~\ref{line:if-random} of the algorithm \textsc{OptimalOmissionsConsensus} as the ratio of $1$'s of operative processes to all values is always either $0$ or $1$. Consequently, the probability that after all such triples, the operative processes do not have the same value in variable $b$ is at most $\frac{1}{n^{C}}$, for some absolute constant $C > 0$. 

From the previous consideration we get, that with probability at least $1 - \frac{1}{n^{C}}$ all operative processes have the same value in the variable $b$ when line~\ref{line:good-spread} of \textsc{OptimalOmissionsConsensus} is executed. 
Since there is at least $\frac{47}{64}n$ operative processes and at most $t  < \frac{1}{192}n$ faulty processes, thus in the next round each non-faulty process receives the value of at least one operative processes and in result adopts the value as its decision. This gives correctness and validity. The termination follows immediately from the fact that the number of epochs, and thus rounds, is fixed.

To estimate the time complexity, we observe that each epoch takes $3 + 4\log{n}$ rounds. Having $\sqrt{n} \cdot \log{n}$ such epochs leads to $O\left(\sqrt{n} \log^2{n}\right)$ rounds in total.

To upper bound bit complexity, we first analyze how many bits are sent per epoch. 
The algorithm \textsc{GroupBitsAggregation} uses $O(n\log^2{n})$ bits per group as it is given in Lemma~\ref{lem:msg-aggr}. Since the algorithm is executed in parallel on $\ceil{\sqrt{n}}$ groups, this results in $O(n^{3/2} \log^{2}{n})$ bits per call of the algorithm.
The algorithm \textsc{GroupBitsSpreading} takes $O(\log{n})$ rounds of communication on a random graph with a degree $O(\log{n})$ at most, with high probability, according to Theorem~\ref{thm:random-graph-properties}. Per each link of the communication graph, processes send at most $O(\sqrt{n}\log{n})$ bits, amortized -- each process sends in a round only this information that has not been passed yet and the total number of information corresponding to the size of the array $\texttt{BitPacks}$, which can be $O(\sqrt{n}\log{n})$ bits at most. 
Since there are $O(\sqrt{n}\log{n})$ epochs, thus the claimed communication complexity follows.
%
\end{proof}
%}


==> src/combinatorial_properties.tex <==
\subsubsection{Combinatorial structure of random regular graphs}
Let $\alpha$, $\beta$, $\delta$, $\gamma$ and~$\ell$ be positive integers and $0< \varepsilon <1$ be a real number.
The following definition extends the notion of a lower bound on a node degree:

\BB
\begin{description}
\item[\em Dense neighborhood:]
For a node $v\in V$, a set $S\subseteq N^{\gamma}_G(v)$  is said to be \emph{$(\gamma,\delta)$-dense-neighborhood for~$v$} if each node in~$S\cap N^{\gamma-1}_G(v)$ has at least $\delta$ neighbors in~$S$.
\end{description}

\BB
\noindent
We want our overlay graphs to have the following properties, for suitable parameters $\alpha$, $\beta$, $\delta$~and~$\ell$:

\BB
\begin{description}

\B
\item[\em Expansion:]
graph~$G$ is said to be  \emph{$\ell$-expanding}, or to be an \emph{$\ell$-expander}, if any two subsets of~$\ell$ nodes each are connected by an edge.
\B
\item[\em Edge-density:]
graph~$G$ is said to be \emph{$(\ell,\alpha,\beta)$-edge-dense} if, for any set $X\subseteq V$ of \emph{at least} $\ell$ nodes, there are at least $\alpha |X|$ edges internal for~$X$, and for any set $Y\subseteq V$ of \emph{at most} $\ell$ nodes, there are at most $\beta |Y|$ edges internal for~$Y$.
\B			
\item[\em Compactness:]
graph~$G$ is said to be \emph{$(\ell,\varepsilon,\delta)$-compact} if, for any set $B\subseteq V$ of at least $\ell$ nodes, there is a subset $C \subseteq B$ of at least $\varepsilon\ell$ nodes such that 
each node's degree in~$G|_C$ is at least~$\delta$. 
We call any such set~$C$ a \emph{survival set for~$B$}.
\end{description}

\BB

%TODO precise the lemma below, esp (n / 192)
\begin{lemma}\label{lemma:random-graph-properties}
For $n \in \textbf{N}$, $k := \frac{2}{3}n$ and $\delta := 36\log{n}$,	a random graph $G_{n, \delta}$ satisfies all the below properties whp:\\
\noindent  
	\emph{(i)} it is $(n/192)$-expanding, 
\hspace*{4.8em}
	\emph{(ii)} it is $(n/96,3/4,\delta/36)$-compact, 

\noindent	\emph{(iii)} it is $(n/96,\delta/8,\delta/144)$-edge-dense,
\hspace*{0.5em}
%	\emph{(iv)} the degree of each node is between $22\frac{n}{k}\delta$ and $26\frac{n}{k}\delta$.
	
\noindent	\emph{(v)} if $\lambda_{1} \ge \lambda_{2} \ge \ldots \ge \lambda_{n}$ are eigenvalues of its normalized adjacency matrix, then $|\max(\lambda_{2}, \lambda_{n}) | \le \frac{1}{\sqrt{\delta}}.$\footnote{https://web.mit.edu/18.338/www/2012s/projects/yz\_slides.pdf}
\end{lemma}

\begin{lemma}[\cite{CK-PODC09}] \label{lemma:sparse-to-dense}		
If graph~$G=(V,E)$ of $n$ nodes is $(n/96,\delta/8,\delta/144)$-edge-dense then any $(r,\delta/36)$-dense-neighborhood for a node $v\in V$ has at least $\min\{2^{r}, n/96\}$ nodes, for $r \ge 0$.
\end{lemma}

\begin{lemma}
Let $G'$ be an subgraph\footnote{Note, that it does not have to be induced subgraph!} of graph $G_{n, \delta}$ satisfying the following list of properties:
\\ \noindent $\textit{(i)}$ $|G'| \ge C_{1} \cdot n,$ for some absolute constant $C_{1}$.
\\ \noindent $\textit{(ii)}$ for every vertex $v \in G'$ and $r \le \log{n / 96}$ there exists a $(r, \delta/36)$-dense-neighborhood of $v$ that is a subbgraph of $G'$.
\\ \noindent $\textit{(iii)}$ at most $n / 400$ vertices have different degrees in $G'$ and $G$. \\
Then the conductance $\Phi(G')$ of the graph $G'$ satisfies:
$$\Phi(G') = \Omega\left(\frac{1}{\delta}\right).$$
\end{lemma}

==> src/new_results.tex <==
\section{Our Results and Technical Novelty}

%In this work, we present a lower bound on the tradeoff between time and use of randomization for Consensus algorithms under omission failures, followed by three new algorithms.
%We compare our results to the previous ones and discuss other closely related work.
%The summary is given in Table~\ref{tab:our_results}.
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
     \hline
     &
     result & time & comm. bits & random bits & comments \\
     \hline
     \hline
%     algo- & \cite{DolevS83} & $O\left(t+1 \right)$ & $O\left(n t \right)$ & 
%     none & $t<n/2$ \\     
     algo- 
     & 
     \underline{Thm~\ref{thm:omissions-opt-res}}
     & $O\left(\frac{t}{\sqrt{n}}\log^2{n} \right)$ & $O(n(t \log^{4}n 
      + n ) )$ 
     & 
     $O\left(t\sqrt{n}\log^2{n} \right)$ & $t \le \frac{n}{192}$\\
%
%     rithms & 
%     & & $ + n ) )$ & 
%     & \\

     rithms 
     &
    \underline{Thm~\ref{thm:trade-off-res}}
%    Theorem~\ref{thm:trade-off-res} 
    & $O\left(\frac{n^{2}}{R}\log^2{n}\right)$ & $O\left(n^2\log^5{n}\right)$ & $O\left(R\log^2{n}\right)$ & $\forall R \in O\left(n^{3/2}\right)$\\
     \hline
     lower & \cite{Bar-JosephB98} & 
     $\Omega\left(\frac{t}{\sqrt{n\log n}} \right)$ 
     & - & - & corr. prob. $= 1$\\
     bounds & \cite{AbrahamCDNPRS19} & - & $\Omega\left(\epsilon t^2\right)$ & - & corr. prob. $\ge \frac{3}{4} + \epsilon$\\
      & 
     \underline{Thm~\ref{thm:lower-randomness-res}}
     & $T$ & - & $R$ & $T\times (R+T) = \Omega\left(\frac{t^2}{\log{n}}\right)$ \\
     & 
     
     &  &  &  & corr. prob. $\ge 1 - \frac{1}{n^{3/2}}$ \\
     \hline
     %\hline
     %notes & \multicolumn{2}{l}{$a, \epsilon \in (0,1)$ - some constants} & %\multicolumn{1}{l}{$c, \varepsilon \in (0,1)$ - any const.} 
     %& \multicolumn{2}{l|}{$\log^{(3)}n = \log\log\log{n}$} \\
     %\hline
\end{tabular}
\caption{Our main results presented for three metrics: time complexity, total number of used communication bits and total number of used random bits. All our algorithms are subject to their complexity bounds whp. 
The parameter $t$ denotes the upper bound on the number of omission-faulty processes, while $n$ is the number of all processes. $T$ and $R$ are random variables denoting, respectively, the number of rounds and the cumulative number of accesses to a random source by all processes in a run of an algorithm. The last two lower bounds are proven for a wider class of algorithms, including not only those correct with probability $1$ but also some other with certain correctness probability smaller than $1$. The references to the results of this paper are underlined.
\label{tab:our_results}}
\end{table}

%\subsection{Lower bound on tradeoff between time and amount of randomization}


%Using this tool and analyzing valency of the executions, which is a generic framework used in related contexts (c.f.~\cite{Bar-JosephB98, Aspnes98, DBLP:conf/stoc/AttiyaC07}), we obtain an amortized analysis while enforcing a time lower bound. However, we use much tighter techniques on the way, taking into account the number of accesses to random sources, c.f., Lemmas~\ref{lem:null-valent} and~\ref{lem:bi-valent}, and their amortized number when classifying states according to their valency, c.f., the conditions defining the valency types of states.


%\noindent 
%\textbf
%\Paragraph{Consequences of the lower bound.}


\subsection{Consensus algorithms}
Focusing on the omissions failures, we present an algorithm that is simultaneously almost-optimal\footnote{
Recall that in this work, almost-optimal means optimal with respect to a poly-logarithmic factor.} 
with respect to time, communication bit and randomness complexities against the most powerful adaptive adversary. The algorithm introduces a novel partitioning of processes into operative and inoperative groups, based on the communication received by each process, which is independent from the standard classification into faulty / non-faulty ones. In this way, faulty processes either communicate well enough to contribute to progress towards a unified decision or become excluded from the set of operative processes, having no impact on the final decision. On a technical level, we demonstrate how to manage the set of operative processes (which may now include faulty ones) without increasing the communication complexity while keeping the round complexity low, and how to use the estimated outcome computed by them to reach agreement.

\begin{theorem}
\label{thm:omissions-opt-res}
There exists an algorithm solving Consensus (with probability~$1$) against the %most powerful 
adaptive adversary that may cause message omissions in $t \le \frac{n}{192}$ processes, which, whp, terminates in $O\left(\frac{t}{\sqrt{n}}\log^{2}{n}\right)$ rounds and uses, in total, $O(n(t \log^{4}n + n ) )$ bits of communication and $O\left(t\cdot \sqrt{n}\log^{2}{n}\right)$
%$O\left(t\cdot n\log^{2}{n}\right)$ 
bits of randomness.
\end{theorem}


The almost-optimal running time and randomness complexity follows from Theorem~\ref{thm:lower-randomness-res}. Recently, Abraham et al.~\cite{AbrahamCDNPRS19} showed that any (even randomized) algorithm that solves Consensus with a constant probability against the adaptive omission-causing adversary requires $\Omega(t^2 + n)$ messages.
Theorem~\ref{thm:omissions-opt-res} shows that the result is almost-tight for $t = \Theta\left(n\right)$. The pseudocode of the algorithm and 
the
%a rigorous 
proof of Theorem~\ref{thm:omissions-opt-res} are given in Section~\ref{sec:main-algo}.

%\noindent \textbf
%\Paragraph
\subsubsection{Algorithm trading time for randomness}

==> src/previous-related.tex <==
\subsection{Previous and Related Work}
\label{sec:related}

\paragraph{Consensus in the classic (non-quantum) model.}
%Classic consensus against an {\em adaptive adversary}.}


%Consensus against an adaptive adversary, considered in this paper, has been already known as more expensive than against weaker adversaries.
Bar-Joseph and Ben-Or~\cite{Bar-JosephB98} proved a lower bound $O(\frac{\sqrt{n}}{\log{n}})$ on expected time complexity of consensus against an adaptive adversary.
They also complemented it by time-optimal randomized algorithm. 
%to the consensus problem was given by Bar-Joseph and Ben-Or~\cite{Bar-JosephB98}. 
Their algorithm uses expected $O(\frac{n^{3/2}}{\log{n}})$ number of communications bits, amortized per process, which has been recently improved by Hajiaghay, Kowalski and Olkowski~\cite{HKO-STOC-2022} to $O(\sqrt{n})$ (while maintaining the almost-optimal round complexity $O(\sqrt{n}\log{n})$).

Fisher and Lynch~\cite{FL} proved a lower bound $f+1$ on {\em deterministic} consensus with $f$ crashes, thus separating deterministic solutions from randomized.
%that deterministic synchronous solution requires $f+1$ rounds if up to~$f$~processes~may~crash.
Regarding communication complexity, Amdur, Weber and Hadzilacos~\cite{AWH} showed that 
%$\Omega(n)$ messages need to be sent by a protocol solving consensus in an eventually synchronous environment in a failure-free execution; hence, 
the amortized number of messages
%communication bits 
per process is at least constant,
even in some failure-free execution.
%
Dwork, Halpern and Waarts~\cite{DHW} found a solution with $\cO(\log n)$ messages per process, but requiring an exponential time, and later Galil, Mayer and Yung~\cite{GMY} developed a message-optimal algorithm working in over-linear $\cO(n^{1+\varepsilon})$ time, for any $0<\varepsilon<1$.
%with $\cO(n)$ messages, thus showing that this amount of messages is optimal.
%The drawback of the latter solution is that it runs in an over-linear $\cO(n^{1+\varepsilon})$ time, for any $0<\varepsilon<1$.
They also improved the communication further to a constant number of communication bits per process,
%$O(n)$ bits, 
but the resulting algorithm was exponential in the number of rounds.
%Galil, Mayer and Yung~\cite{GMY} found an early-stopping solution with $\cO(n+fn^\varepsilon)$ communication complexity, for any $0<\varepsilon<1$.
Chlebus and Kowalski~\cite{CK} showed that consensus can be
solved in  $\cO(f+1)$ time and with $\cO(\log^2 f)$ messages
if only the number $n-f$ of non-faulty processors satisfies $n-f=\Omega(n)$.
It was later improved in~\cite{CK-PODC09} to $O(f)$ time and $O(\polylog n)$ number of communication bits.
%The time complexity $f+1$ is optimal for consensus, as shown by Fischer and Lynch~\cite{FL}.
%To summarize, when the number of crashes $f$ could be 
%as large as a fraction of 
%close to $n$, 
%}%
%The best deterministic algorithm, given by Chlebus, Kowalski and Strojnowski in \cite{CK-PODC09}, solves consensus in asymptotically optimal time
%the time complexity of deterministic consensus is 
%$\Theta(n)$ and an amortized number of communication bits per process $O(\polylog n)$.
All the abovementioned communication complexities are amortized per process.

\Paragraph{Quantum consensus.} To the best of our knowledge, almost all previous papers on quantum consensus concentrated on assuring feasibility of the problem against strong Byzantine adversaries or asynchronous setting, for which no classical solution exists, c.f.,~\cite{Helm-PODC08,LFZ-Physics19}, or on optimizing time complexity, including the work of Ben-Or and Hassidim~\cite{Ben-OrH05} achieving constant time against an adaptive adversary.
%
Sparse quantum communication has been considered by Chlebus, Kowalski and Strojnowski in~\cite{ChlebusKS10}, but their protocols work correctly only with some probability smaller than $1$ and for a specific number of failures corresponding to the probability of success.
Other distributed computing problems, not necessarily fault-prone, were also analyzed in quantum models, c.f.,~\cite{BT-SIGACT08,TKM-TALG12}.

\Paragraph{More efficient classic randomized solutions against {\em weak adversaries}.}

Whenever weaker oblivious adversaries are considered,
randomness itself occurred to be enough in reducing time complexity to a constant. 
%However, whenever randomness is considered, different types of an adversary generating failures could be considered. 
%Message complexity of consensus was extensively studied before. 
%Amdur, Weber and Hadzilacos~\cite{AWH} showed that $\Omega(n)$ messages need to be sent by a protocol solving consensus in an eventually synchronous environment in a failure-free execution.
Chor, Merritt and Shmoys~\cite{CMS} developed constant-time algorithms for consensus against an {\em oblivious adversary} -- that is, the adversary who knows the algorithm but has to decide which process fails and when before the execution starts.
%
%
Their solution, however, requires a linear number of communication bits per process.
Gilbert and Kowalski~\cite{GK-SODA-10} presented a randomized consensus algorithm that achieves optimal communication complexity of $O(1) $ amortized communication bits per process 
%(amortized) 
while terminating in 
$O(\log n) $ time with high probability (whp for short), as long as the number of crashes $ f < n/2 $. 
%against an oblivious adversary.


\Paragraph{Classic consensus in more demanding models.} 
%and/or Counting (gossip?) ???}

%It was shown that more severe failures or asynchrony %or restricted underlying communication networks, 
%could cause a substantially higher complexity.
Dolev and Reischuk~\cite{DR} and Hadzilacos and Halpern~\cite{HH} proved the $\Omega(f)$ lower bound on the amortized message complexity per process %(amortized) 
of deterministic consensus for {\em omission or (authenticated) Byzantine failures}. 
%
However, under some limitation on the adversary and requiring termination only whp, the sublinear expected communication complexity $O(\sqrt{n}\; \polylog{n})$ per process can be achieved even in case of Byzantine failures, as proved by King and Saia~\cite{KingS11}.
%
Such limitations are apparently necessary
to achieve
subquadratic time complexity for Byzantine failures, c.f., Abraham et al.~\cite{AbrahamCDNP0S19}.
%
{\em Asynchrony} also implies large communication --
Aspnes~\cite{Aspnes-JACM-98} proved a lower bound $\Omega(n/\log^2 n)$ on communication complexity per process.
Alistarh, Aspnes, King and Saia~\cite{AlistarhAKS18} showed the most efficient up to date consensus algorithm achieving communication complexity $O(n\log{n})$ per process (amortized) if less then $n/2$ processes may fail. 
%which improved upon the previous result $O(n\log^2 {n})$ by Aspnes and Waarts~\cite{AspnesW-SICOMP-96} and is asymptotically almost optimal due to the lower bound $\Omega(n/\log^2 n)$ by .
























\remove{%%%%%%%%%%  START  REMOVE  %%%%%%%%%%%%%%%%%%%%%%

\FFF
\Paragraph{Early work on consensus.}
%\hspace*{-1em}
The \emph{Consensus} problem was introduced by Pease, Shostak and Lamport~\cite{PSL}.
Early work focused on {\em deterministic} solutions.
Fisher, Lynch and Paterson~\cite{FLP} showed that the problem is unsolvable in an asynchronous setting, even 
if one process may fail.
Fisher and Lynch~\cite{FL} showed that a synchronous solution requires $f+1$ rounds if up to~$f$~processes~may~crash.


%\paragraph{Consensus in crash-prone message-passing system.}

The optimal complexity of consensus with crashes is known with respect to the time and the number of messages (or communication bits) when each among these performance metrics is considered separately. 
Amdur, Weber and Hadzilacos~\cite{AWH} showed that 
%$\Omega(n)$ messages need to be sent by a protocol solving consensus in an eventually synchronous environment in a failure-free execution; hence, 
the amortized number of messages
%communication bits 
per process is at least constant,
even in some failure-free execution.
\remove{%
%The lower bound~$\Omega(n)$ on the number of messages clearly holds, c.f.,~\cite{AWH}.
Dwork, Halpern and Waarts~\cite{DHW} found a solution with $\cO(n\log n)$ messages but requiring an exponential time, and later
Galil, Mayer and Yung~\cite{GMY} developed an algorithm with $\cO(n)$ messages, thus showing that this amount of messages is optimal.
The drawback of the latter solution is that it runs in an over-linear $\cO(n^{1+\varepsilon})$ time, for any $0<\varepsilon<1$.
They also improved the communication to $O(n)$ bits, but the resulting algorithm was exponential in the number of rounds.
%Galil, Mayer and Yung~\cite{GMY} found an early-stopping solution with $\cO(n+fn^\varepsilon)$ communication complexity, for any $0<\varepsilon<1$.
Chlebus and Kowalski~\cite{CK} showed that consensus can be
solved in  $\cO(f+1)$ time and with $\cO(n\log^2 f)$ messages
if only the number $n-f$ of non-faulty processors satisfies $n-f=\Omega(n)$.
It was later improved in~\cite{CK-PODC09} to $O(f)$ time and $O(n\; \polylog n)$ number of communication bits.
%The time complexity $f+1$ is optimal for consensus, as shown by Fischer and Lynch~\cite{FL}.
To summarize, when the number of crashes $f$ could be 
%as large as a fraction of 
close to
$n$, 
}%
The best deterministic algorithm, given by Chlebus, Kowalski and Strojnowski in \cite{CK-PODC09}, solves consensus in asymptotically optimal time
%the time complexity of deterministic consensus is 
$\Theta(n)$ and an amortized number of communication bits per process $O(\polylog n)$.

\Paragraph{Efficient randomized solutions against {\em weak adversaries}.}

Randomness proved itself useful to break a linear time barrier for time complexity. 
However, whenever randomness is considered, different types of an adversary generating failures could be considered. 
%Message complexity of consensus was extensively studied before. 
%Amdur, Weber and Hadzilacos~\cite{AWH} showed that $\Omega(n)$ messages need to be sent by a protocol solving consensus in an eventually synchronous environment in a failure-free execution.
Chor, Merritt and Shmoys~\cite{CMS} developed constant-time algorithms for consensus against an {\em oblivious adversary} -- i.e., the adversary who knows the algorithm but has to decide which process fails and when before the execution starts.
%
%
Gilbert and Kowalski~\cite{GK-SODA-10} presented a randomized consensus algorithm that achieves optimal communication complexity, using $ \mathcal{O}(1) $ amortized communication bits per process 
%(amortized) 
and terminates in 
$ \mathcal{O}(\log n) $ time with high probability, tolerating up to $ f < n/2 $ crash failures. 
%against an oblivious adversary.


\Paragraph{Randomized solutions against (strong) {\em adaptive adversary}.}
Consensus against an adaptive adversary, considered in this paper, has been already known as more expensive than against
%comparing to 
weaker adversaries.
The time-optimal randomized solution to the consensus problem was given by Bar-Joseph and Ben-Or~\cite{Bar-JosephB98}. Their algorithm works in $O(\frac{\sqrt{n}}{\log{n}})$ expected time and uses $O(\frac{n^{3/2}}{\log{n}})$ amortized communications bits per process, %(amortized), 
in expectation. 
They also proved 
%the 
optimality of their result with respect to the time complexity, while 
here we substantially improve the communication.


\Paragraph{Beyond synchronous crashes.}
It was shown that more severe failures or asynchrony %or restricted underlying communication networks, 
could cause a substantially higher complexity.
Dolev and Reischuk~\cite{DR} and Hadzilacos and Halpern~\cite{HH} proved the $\Omega(f)$ lower bound on the amortized message complexity per process %(amortized) 
of deterministic consensus for {\em (authenticated) Byzantine failures}. 
%
King and Saia~\cite{KingS11} proved that under some limitation on the adversary and requiring termination only whp, the sublinear expected communication complexity $O(n^{1/2}\polylog{n})$ per process can be achieved even in case of Byzantine failures. 
%
Abraham et al.~\cite{AbrahamCDNP0S19} showed necessity of such limitations 
to achieve
subquadratic time complexity for Byzantine failures.

If {\em asynchrony} occurs, the recent result of Alistarh
%, Aspnes, King and Saia
et al.~\cite{AlistarhAKS18} showed how to obtain almost optimal communication complexity $O(n\log{n})$ per process (amortized) if less then $n/2$ processes may fail, which improved upon the previous result $O(n\log^2 {n})$ by Aspnes and Waarts~\cite{AspnesW-SICOMP-96} and is asymptotically almost optimal due to the lower bound $\Omega(n/\log^2 n)$ by Aspnes~\cite{Aspnes-JACM-98}.
%in message-passing networks. 
%Interestingly, the result in~\cite{AlistarhAKS18} uses different approach, which is focused on reducing the asynchrony side effects rather than providing sparse communications graphs, as in our case.


\Paragraph{Efficient Fault-tolerant Counting} 
was introduced by Hajiaghay, Kowalski and Olkowski~\cite{HKO-STOC-22}.
Gossip was introduced by Chlebus and Kowalski~\cite{CK}.
They developed a deterministic algorithm solving %\emph{Gossip-with-Crashes} 
Gossip
in time $\cO(\log^2 f)$ while using $\cO(\log^2 f)$ amortized messages per process, provided $n-f=\Omega(n)$.
They also showed a lower bound  $\Omega(\frac{\log n}{\log(n\log n)-\log f})$ on the number of rounds
in case $\cO(\polylog n)$ amortized messages are used per process.
%
In a sequence of papers~\cite{CK,GKS,CK-DISC06},
$O(\polylog n)$ message complexity, amortized per process, was obtained for any $f<n$, while keeping the polylogarithmic time complexity.
%improved to  in \cite{CK-DISC06}.
Note however that general Gossip requires $\Omega(n)$ communication bits per process for different rumors, as each process needs to deliver/receive at least one bit to all non-faulty processes.
%
%\JOO{
Randomized gossip 
%in a synchronous systems 
against an adaptive adversary is doable
%in such environment there 
%it is possible to achieve Gossip 
w.h.p. in $O(\log^{2}{n})$ rounds 
using $O(\log^{3}{n})$ communication bits per process, for a constant number of rumors of constant size and for $f < \frac{n}{3}$ processes, c.f.,
Alistarh et al.~\cite{AlistarhGGZ10}.
%even if the failures are adaptive. 
%
%In their protocol processes need to have unique names only, while the assumption that every process knows names of other processes is relaxed.
%A similar technique 
%however 
%extended to any aggregation function calculated on the set of all non-faulty processes beside the accumulating function, 
%and its practical evaluations, 
%was used by Gupta et al.~\cite{GuptaRB01}
%to calculate aggregation~functions.
%}

\Paragraph{Other quantum consensus results.}
\dk{??? SHOULD WE PUT ANY RELATED WORK, MOSTLY ON BYZANTINE ???}

\remove{A graph is said to be \emph{$\ell$-expanding}, or to be an \emph{$\ell$-expander}, if any two subsets of~$\ell$ nodes each are connected by an edge; this notion was first introduced by Pippenger~\cite{Pip}.
	%	Observe that $(\ell,\alpha,\beta)$-edge-expansion implies the $\ell$-expanding property for $\alpha>0$.
	%	In our algorithm we will use $\ell$-expanders for $\ell=n/2^i$ and for $\ell=(2/3)^i n/64$, for $i\ge 1$.
	There exist $\ell$-expanders  of the maximum degree $\cO(\frac{n}{\ell}\log n)$, as can be proved by the probabilistic method; such an argument was first used by Pinsker~\cite{Pin}. 
}

}
